Operator Fusion in XLA: Analysis and Evaluation

Machine learning (ML) compilers are an active area of research because they offer the potential to automatically speedup tensor programs. Kernel fusion is often cited as an important optimization performed by ML compilers. However, there exists a knowledge gap about how XLA, the most common ML compiler, applies this nuanced optimization, what kind of speedup it can afford, and what low-level effects it has on hardware. Our paper aims to bridge this knowledge gap by studying key compiler passes of XLA's source code. Our evaluation on a reinforcement learning environment Cartpole shows how different fusion decisions in XLA are made in practice. Furthermore, we implement several XLA kernel fusion strategies that can achieve up to 10.56x speedup compared to our baseline implementation.

==> motivation.tex <==
\section{Motivation}
\textcolor{red}{this section can be removed.}

Our project is motivated by the lack of public documentation about the optimizations performed by XLA \cite{XLA}. What optimizations does XLA perform (or not)? The XLA documentation states that kernel fusion is the "single most important optimization" \cite{XLA_web}, however it is still not clear how kernel fusion is implemented in XLA. No papers explore the trade-offs in XLA's kernel fusion. We also believe that because XLA has been developed with a focus on TPU accelerator hardware, and that there exists a large space to propose new XLA optimizations for GPU kernel fusion. 

The XLA kernel fusion C++ source code \cite{XLA_fusion_code} is short, well written, and approachable, but beyond that no documentation or explanation of XLA's kernel fusion decisions exist. Filling this knowledge gap will be our primary contribution. We will study the trade-offs in XLA as well as in its kernel fusion decision making process. 

Our second contribution will be to implement our best idea in XLA's kernel fusion codebase and seek potential speedup in some important benchmarks. We also hope that our implementation will be merged into the XLA code base.
